Density Sketches for Sampling and Estimation

We introduce Density sketches (DS): a succinct online summary of the data distribution. DS can accurately estimate point wise probability density. Interestingly, DS also provides a capability to sample unseen novel data from the underlying data distribution. Thus, analogous to popular generative models, DS allows us to succinctly replace the real-data in almost all machine learning pipelines with synthetic examples drawn from the same distribution as the original data. However, unlike generative models, which do not have any statistical guarantees, DS leads to theoretically sound asymptotically converging consistent estimators of the underlying density function. Density sketches also have many appealing properties making them ideal for large-scale distributed applications. DS construction is an online algorithm. The sketches are additive, i.e., the sum of two sketches is the sketch of the combined data. These properties allow data to be collected from distributed sources, compressed into a density sketch, efficiently transmitted in the sketch form to a central server, merged, and re-sampled into a synthetic database for modeling applications. Thus, density sketches can potentially revolutionize how we store, communicate, and distribute data.

==> res.tex <==
\begin{table}
\begin{tabular}{|l|l|l|l|}
\hline
Dataset                                                     & Dimension & Samples & zipped size \\ \hline
skin/nonskin                                                & 3         & 180K    & 670KB       \\ \hline
susy                                                        & 18        & 4.5M    & 0.8GB       \\ \hline
higgs                                                       & 28        & 10M     & 2.5GB       \\ \hline
\begin{tabular}[c]{@{}l@{}}webspam\\ (unigram)\end{tabular} & 254       & 300K    & 120MB       \\ \hline
\end{tabular}
\caption{Classification Datasets from \cite{liblinear} with dimenstion $< 500$, number of samples per class $> 100,000$}
\label{tab:datasets}
\vspace{-0.2cm}
\end{table}
\begin{figure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/skinA.png}
  \caption{skin/nonskin}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/higgsA.png}
  \caption{higgs }
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/susyA.png}
  \caption{ susy}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/webspamuniA.png}
  \caption{webspam(unigram)}
\end{subfigure}
\caption{\textbf{Classification Results} : Test accuracy of models trained on samples drawn from density sketches and a random sample. Models from Original data are horizontal lines. Datasets chosen as \ref{tab:datasets}. When compared for original accuracy, we get \textbf{$\approx$200x} Compression in "skin", \textbf{$\approx$150x} compression in "susy", \textbf{$\approx$50x} compression in "higgs" with Densiy Sketches}
\label{fig:classification}
\end{figure} 
\begin{figure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/skinC.png}
  \caption{skin/nonskin}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/higgsC.png}
  \caption{higgs }
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/susyC.png}
  \caption{ susy}
\end{subfigure}
\begin{subfigure}{.23\textwidth}
  \centering
  \includegraphics[width=.95\linewidth]{figures/webspamuniC.png}
  \caption{webspam(unigram)}
\end{subfigure}
\caption{\textbf{Estimation Error}: Mean Square Error of the predicted covariance matrix from samples drawn from Density Sketches and Random Sample as compared to the empirical covariance matrix of the original data. Datasets chosen as \ref{tab:datasets}}
\label{fig:estimation}
\end{figure}



==> vis_tab.tex <==
%\begin{figure*}[]
%\includegraphics[scale=0.07]{figures/mgaussian_true.png}
%\includegraphics[scale=0.07]{figures/mgaussian_true.png}
%\includegraphics[scale=0.07]{figures/mgaussian_true.png}
%resizebox{0.2\textwidth}{!}{
%\begin{tabular}{|l|l|l|l|}
%\hline
%Dataset                                                     & Dimension & Samples & zipped size \\ \hline
%skin/nonskin                                                & 3         & 180K    & 670KB       \\ \hline
%susy                                                        & 18        & 4.5M    & 0.8GB       \\ \hline
%higgs                                                       & 28        & 10M     & 2.5GB       \\ \hline
%webspam                                                     & 254       & 300K    & 120MB       \\ \hline
%\end{tabular} }
%
%%\captionlistentry[table]{A table beside a figure}
%    \captionsetup{labelformat=andtable}
%\caption{A table beside a figure}
%\end{figure*}


\begin{table*}
\begin{tabular}{|l|l|l|l|}
\hline
\includegraphics[trim=200 50 200 50 ,clip,width=0.2\textwidth]{figures/mgaussian_true.png} & \includegraphics[trim=200 50 200 50 ,clip,width=0.2\textwidth]{figures/mgaussian_race.png} & \includegraphics[trim=200 50 200 50 ,clip,width=0.2\textwidth]{figures/mnist_sampling.png} & \resizebox{0.25\textwidth}{!}{\begin{tabular}{|l|l|l|l|}
Dataset                                                     & Dimension & Samples & zipped size \\ \hline
skin/nonskin                                                & 3         & 180K    & 670KB       \\ \hline
susy                                                        & 18        & 4.5M    & 0.8GB       \\ \hline
higgs                                                       & 28        & 10M     & 2.5GB       \\ \hline
webspam\\ (unigram)                                         & 254       & 300K    & 120MB       \\ \hline
\end{tabular} } \\ \hline
\end{tabular}
\caption{Classification Datasets from \cite{liblinear} with dimenstion $< 500$, number of samples per class $> 100,000$}
\label{tab:datasets}
\vspace{-0.2cm}
\end{table*}




